Precise Condition Synthesis for Program Repair

Due to the difficulty of repairing defect, many research efforts have been devoted into automatic defect repair. Given a buggy program that fails some test cases, a typical automatic repair technique tries to modify the program to make all tests pass. However, since the test suites in real world projects are usually insufficient, aiming at passing the test suites often leads to incorrect patches. In this paper we aim to produce precise patches, that is, any patch we produce has a relatively high probability to be correct. More concretely, we focus on condition synthesis, which was shown to be able to repair more than half of the defects in existing approaches. Our key insight is threefold. First, it is important to know what variables in a local context should be used in an "if" condition, and we propose a sorting method based on the dependency relations between variables. Second, we observe that the API document can be used to guide the repair process, and propose document analysis technique to further filter the variables. Third, it is important to know what predicates should be performed on the set of variables, and we propose to mine a set of frequently used predicates in similar contexts from existing projects. We develop a novel program repair system, ACS, that could generate precise conditions at faulty locations. Furthermore, given the generated conditions are very precise, we can perform a repair operation that is previously deemed to be too overfitting: directly returning the test oracle to repair the defect. Using our approach, we successfully repaired 17 defects on four projects of Defects4J, which is the largest number of fully automatically repaired defects reported on the dataset so far. More importantly, the precision of our approach in the evaluation is 73.9%, which is significantly higher than previous approaches, which are usually less than 40%.

==> impl.tex <==
\section{Implementation}\label{sec:implementation}
We have implemented our approach as a Java program repair system,
\approach. \approach stands for accurate condition synthesis. 

The fault localization component is implemented by modifying the
source code of
Nopol\footnote{http://github.com/SpoonLabs/nopol/}~\cite{xuan2016nopol}.
More specifically, the spectrum-based fault localization is
implemented using
GZoltar\footnote{http://gzoltar.com/}~\cite{Campos2012GZoltar}, which
is a fault localization library that includes the implementation of
algorithm Ochiai~\cite{abreu2007accuracy}. 
Based on that, we implement
our own predicate switching component, which record more information than
the original Nopol algorithm to support our condition synthesis,
and the condition synthesis component. The invocation of
\url{searchcode.com} is implemented via the web API provided by
searchcode, which allows a continuous query of the results.

In the implementation we also observed and corrected some deficiencies
of the existing tool chains, which are worth noting for future 
implementations of program repair tools.

First, both GZoltar and Nopol treat a test method as a test case.
However, this may not be true in practice. For example, the following
piece of code is a test method for the defect Math-99 from
Defects4J~\cite{martinez2015automatic}. The method under test,
\code{MathUtils.gcd}, is called several times in one test method, enough time with
a different set of test inputs, and its output is compared with a
different test oracle.
\begin{lstlisting}
public void testGcd() {
  ...
  assertEquals(0, MathUtils.gcd(0, 0));
  assertEquals(b, MathUtils.gcd(0, b));
  assertEquals(a, MathUtils.gcd(a, 0));
  ... }
\end{lstlisting}
If we treat all invocations to \code{gcd} as one test case, when any of the
invocations fails to pass the oracle, the whole test case is
considered to fail, though all other invocations actually produce the
expected outputs. As result, the precision of spectrum-based fault
localization is unnecessarily degraded.

Second, GZoltar does not support the code inside a constructor,
leading to being unable to locate all faults inside a constructor.

Our implementation and experimental data are open source and are
available on the web\footnote{The link to repository is removed for double-blind review.}.


% Things to say here: (1) Nopol treats test cases wrongly. (2) glozar
% bug: ignore constructors


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ase16-fix"
%%% End:

